Poly-YOLO: higher speed, more precise detection and instance segmentation for YOLOv3

We present a new version of YOLO with better performance and extended with instance segmentation called Poly-YOLO. Poly-YOLO builds on the original ideas of YOLOv3 and removes two of its weaknesses: a large amount of rewritten labels and inefficient distribution of anchors. Poly-YOLO reduces the issues by aggregating features from a light SE-Darknet-53 backbone with a hypercolumn technique, using stairstep upsampling, and produces a single scale output with high resolution. In comparison with YOLOv3, Poly-YOLO has only 60% of its trainable parameters but improves mAP by a relative 40%. We also present Poly-YOLO lite with fewer parameters and a lower output resolution. It has the same precision as YOLOv3, but it is three times smaller and twice as fast, thus suitable for embedded devices. Finally, Poly-YOLO performs instance segmentation using bounding polygons. The network is trained to detect size-independent polygons defined on a polar grid. Vertices of each polygon are being predicted with their confidence, and therefore Poly-YOLO produces polygons with a varying number of vertices.

==> YOLO v4_rev_1/sections/current_state.tex <==

\subsection{Object detection}
Models for object detection can be divided into two groups, two-stage, and one-stage detectors. Two-stage detectors split the process as follows. In the first phase, regions of interest (RoI) are proposed, and in the subsequent stage, bounding box regression and classification is being done inside these proposed regions. One-stage detectors predict the bounding boxes and their classes at once. Two-stage detectors are usually more precise in terms of localization and classification accuracy, but in terms of processing are slower then one-stage detectors. Both of these types contain a backbone network for feature extraction and head networks for classification and regression. Typically, the backbone is some SOTA network such as ResNet~\cite{he2017mask} or ResNext~\cite{xie2017aggregated}, pre-trained on ImageNet or OpenImages. Even though, some approaches~\cite{shen2019object}, \cite{zhu2019scratchdet} also experiment with training from scratch.

\subsubsection{Two-stage detectors}
The prototypical example of two-stage architecture is Faster R-CNN~\cite{ren2015faster}, which is an improvement of its predecessor Fast R-CNN~\cite{girshick2015fast}. The main improvement lies in the use of Region Proposal Network (RPN), which replaced a much slower selective search of RoIs. It also introduced the usage of multi-scale anchors to detect objects of different sizes. %It is trained using a multi-task loss function, which optimizes four losses at once. Two losses are computed for the proposed RoIs by the RPN where the first is for RoI regression, and the second is for object/background classification of the ROI. Another two losses are computed for the final classification score and final box coordinates. 
Faster R-CNN is, in a way, a meta-algorithm that can have many different incarnations depending on a type of the backbone and its heads. One of the frequently used backbones, called Feature Pyramid Network (FPN)~\cite{dollar2014fast}, allows to predict RoIs from multiple feature maps, each with a different resolution. This is beneficial for the recognition of objects at different scales. 

\subsubsection{One-stage detectors}
Two best-known examples of one-stage detectors are YOLO~\cite{redmon2018yolov3} and SSD~\cite{liu2016ssd}. The architecture of YOLO will be thoroughly described in Section~\ref{sec-yolo}. Usually, one-stage detectors divide the image into a grid and predict bounding boxes and their classes inside them, all at once. Most of them also use the concept of anchors, which are predefined typical dimensions of bounding boxes that serve as apriori knowledge. One of the major improvements in the area of one-stage detectors was a novel loss function call Focal Loss \cite{lin2017focal}. Because of the fact that two-stage detectors produce a sparse set of region proposals in the first step, most of the negative locations are filtered out for the second stage. One-stage detectors, on the other hand, produce a dense set of region proposals which they need to classify as containing objects or not. This creates a problem with the non-proportional frequency of negative examples. Focal Loss solves this problem by adjusting the importance of negative and positive examples within the loss function. 
Another interesting idea was proposed in an architecture called RefineDet~\cite{zhang2018single}, which performs a two-step regression of the bounding boxes. The second step refines the bounding boxes proposed in the first step, which produces more accurate detection, especially for small objects.
Recently, there has been a surge of interest in approaches that do not use anchor boxes. The main representative of this trend is the FCOS framework~\cite{tian2019fcos}, which works by predicting four coordinates of a bounding box for every foreground pixel. These four coordinates represent a distance to the four boundary edges of a bounding box in which the pixel is enclosed in. The predicted bounding boxes of every pixel are subsequently filtered by NMS. Similar anchor-free approach was proposed in CornerNet~\cite{law2018cornernet}, where the objects are detected as a pair of top-left and bottom-right corners of a bounding box.

%GraphNets, NAS, EfficientDet
%Combination of 1 and 2 stage detectors
%SlowFast Networks for Video Recognition

%Pedestrian detection: An evaluation of the state of the art %\cite{dollar2011pedestrian}

%Faster R-CNN \cite{ren2015faster}

%Object detection with discriminatively trained part-based models %\cite{felzenszwalb2009object}

%Fast feature pyramids for object detection \cite{dollar2014fast}

%Object detection in videos by high quality object linking \cite{tang2019object}

%What Makes for Effective Detection Proposals? \cite{hosang2015makes}

%Region-Based Convolutional Networks for Accurate Object Detection and Segmentation \cite{girshick2015region}

%Mask R-CNN \cite{he2017mask}

%Object Detection Networks on Convolutional Feature Maps \cite{ren2017objectdet}



\subsection{Instance Segmentation}
In many applications, a boundary given by a rectangle may be too crude, and we may instead require a boundary framing the object tightly. In the literature, this task is called Instance Segmentation, and the main approaches also fit into the one-stage/two-stage taxonomy. The prototypical example of a two-stage method is an architecture called Mask R-CNN~\cite{he2017mask}, which extended Faster R-CNN by adding a separate fully-convolutional head that predicts masks of objects. Note, the same principle is also applied to RetinaNet, and the improved net is called RetinaMask~\cite{fu2019retinamask}. One of Mask R-CNN innovations is a novel way for extracting features from RoIs using the RoIAlign layer, which avoids the problem of misalignments of the RoI due to its quantization to the grid of the feature map. 
One-stage methods for instance segmentation can be further divided into top-down methods, bottom-up methods, and direct methods. Top-down methods~\cite{chen2019tensormask,bolya2019yolact} work by first detecting an object and then segmenting this object within a bounding box. Prediction of bounding boxes either uses anchors or is anchor free following the FCOS framework~\cite{tian2019fcos}. Bottom-up methods~\cite{newell2017associative,liu2017sgn}, on the other hand, work by first embedding each pixel into a metric space in which are these pixels subsequently clustered. As the name suggests, direct methods work by directly predicting the segmentation mask without bounding boxes or pixel embedding~\cite{wang2020solov2}. We also mention that independently of our instance segmentation, PolarMask~\cite{xie2019polarmask} introduces instance segmentation using polygons, which are also predicted in polar coordinates. In comparison with PolarMask, Poly-YOLO learns itself in general size-independent shapes due to the use of the relative size of a bounding polygon according to the particular bounding box. The second difference is that Poly-YOLO produces a dynamic number of vertices per polygon, according to the shape-complexity of various objects.

%\subsection{Distance estimation}
%The easiest way to estimate an object distance is the usage of an active approach using active devices emitting energy into a scene. However, such approaches need additional, typically expensive hardware. Passive approaches use the image scene captured by camera(s), using depth-map estimation by direct object distance estimation.

%A depth map is mainly estimated by a disparity map produced from two aligned stereo cameras. Generally, disparity-based approaches are quite precise~\cite{mrovlje2008distance}; the weak point is it's producing. For that, non-neural network approaches are also quite slow, but can be hard-wired on FPGA arrays~\cite{ambrosch2007hardware} to drastically improve the performance. \color{red}(Prepsano vojtou, marek zkontrolovat): The stereo object matching used for further disparity evaluation is an important research topic in the field of "Stereo matching"~\cite{manueldisparity}. \color{black}
%The distance can also be estimated directly using NN. In~\cite{haseeb2018disnet}, the author proposes to combine the YOLO detector and DisNet -- distance estimation neural network processing stereo input images to estimate objects distance. Similar approaches can also be found in~\cite{sattar2019human}, where YOLO is used too. Unfortunately, authors evaluate distance only for pedestrians. \color{red}PREPSAT: Custom CNN for distance estimation~\cite{eigen2014depth}, but not very precise; or MonoDepth CNN~\cite{godard2017unsupervised} with a novel idea of a NN with unsupervised learning producing interesting results.\color{black}

%TODO dopsat z časopisu, dopsat  line lanes

==> YOLO v4_rev_1/sections/graph_nr_of_anchors.tex <==
\noindent
\begin{figure*}[!h]
\vspace{5mm}
\small
\begin{tikzpicture}
      \begin{axis}[
        height=35mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Number of anchors},
        ymin=0,
        ymax=12,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={1, 3, 6, 9, 12, 15, 18},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(1,7.1)(3,6.9)(6,6.8)(9,6.9)(12,7.0)(15,7.0)(18,7.2)};\addlegendentry{Loss~~~~}
        \addplot[fill=orange!40!white]coordinates{(1,8.2)(3,8.0)(6,7.7)(9,7.8)(12,8.0)(15,7.9)(18,8.0)};\addlegendentry{Val loss}
      \end{axis}
    \end{tikzpicture}
~
 \begin{tikzpicture}
      \begin{axis}[
        height=35mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Number of anchors},
        ymin=0,
        ymax=0.1,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={1, 3, 6, 9, 12, 15, 18},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(1,0.064)(3,0.052)(6,0.069)(9,0.069)(12,0.071)(15,0.062)(18,0.051)};\addlegendentry{Box mAP~~~~}
        \addplot[fill=orange!40!white]coordinates{(1,0.057)(3,0.047)(6,0.063)(9,0.062)(12,0.064)(15,0.057)(18,0.047)};\addlegendentry{Mask mAP}
      \end{axis}
    \end{tikzpicture}
    \vspace{-3mm}
\caption{Left: Dependence of number of anchors on loss. Right: Dependence of number of anchors on mAP. Here, 24 vertices are used.}
\label{graph-nr-anchors}
\end{figure*}

==> YOLO v4_rev_1/sections/graph_nr_of_vertices.tex <==
\noindent
\begin{figure*}[!h]
\small
\begin{tikzpicture}
      \begin{axis}[
        height=39mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Maximal number of vertices per polygon},
        ymin=0,
        ymax=12,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={8, 12, 18, 24, 36, 60, 90},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(8,5.4)(12,5.8)(18,6.5)(24,6.9)(36,7.7)(60,8.8)(90,9.6)};\addlegendentry{Loss~~~~}
        \addplot[fill=orange!40!white]coordinates{(8,6.5)(12,6.9)(18,7.5)(24,7.8)(36,8.5)(60,9.5)(90,10.3)};\addlegendentry{Val loss}
      \end{axis}
    \end{tikzpicture}
~
\begin{tikzpicture}
      \begin{axis}[
        height=39mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Number of anchors},
        ymin=0,
        ymax=12,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={1, 3, 6, 9, 12, 15, 18},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(1,7.1)(3,6.9)(6,6.8)(9,6.9)(12,7.0)(15,7.0)(18,7.2)};\addlegendentry{Loss~~~~}
        \addplot[fill=orange!40!white]coordinates{(1,8.2)(3,8.0)(6,7.7)(9,7.8)(12,8.0)(15,7.9)(18,8.0)};\addlegendentry{Val loss}
      \end{axis}
    \end{tikzpicture}
    \vspace{-3mm}
\caption{Left: Dependence of number of vertices on loss for 9 used anchors. Right: Dependence of number of anchors on loss for 24 used vertices.}
\label{graph-nr-vertices}
\end{figure*}

==> YOLO v4_rev_1/sections/graph_se_type.tex <==
\noindent
\begin{figure}[!h]
\begin{tikzpicture}
\small
\begin{axis}[height=40mm,width=98mm,xlabel={Epoch},xmin=10, xmax=50, ymin=6.7,ymax=13,legend style={at={(0.79,1)},anchor=north, nodes={scale=0.9, transform shape}},legend columns=1, ymajorgrids=true,yminorgrids=true,style={ultra thick},axis x line*=bottom, axis y line*=left, legend cell align={left}]
\addplot[green]coordinates{(1,269.1180581)(2,28.21265573)(3,18.40226598)(4,16.42302675)(5,15.21275809)(6,14.13723531)(7,13.14906785)(8,12.39609316)(9,11.69206872)(10,11.11319239)(11,10.64653439)(12,10.21312326)(13,9.90192655)(14,9.567035707)(15,9.401223558)(16,9.163649295)(17,8.925355853)(18,8.807712996)(19,8.657624128)(20,8.591970632)(21,8.452182244)(22,8.28339433)(23,8.239628017)(24,8.149788473)(25,8.107046533)(26,7.95557965)(27,7.836849302)(28,7.81011553)(29,7.697173212)(30,7.641633639)(31,7.646899995)(32,7.605880239)(33,7.543636947)(34,7.46002098)(35,7.466055063)(36,7.349977418)(37,7.27898359)(38,7.269490557)(39,7.147420347)(40,7.09822743)(41,7.108537794)(42,7.081504741)(43,7.037955232)(44,7.043813616)(45,7.017336998)(46,7.006936838)(47,6.996316055)(48,6.937507799)(49,6.924841831)(50,6.897511486)};\addlegendentry{loss of SE-Standard}
%\addplot[green,dashed]coordinates{(1,47.50182178)(2,30.68728327)(3,19.68424953)(4,18.29376094)(5,15.03333042)(6,15.33791863)(7,12.89367659)(8,12.2843216)(9,11.94397123)(10,11.56019573)(11,10.73157223)(12,10.5044645)(13,10.12754359)(14,10.38881053)(15,9.809634464)(16,9.612795427)(17,9.718599434)(18,9.197471745)(19,9.753666145)(20,9.072291718)(21,9.236122705)(22,8.766421022)(23,8.788898129)(24,8.958717487)(25,9.128627947)(26,8.551600418)(27,8.563221022)(28,8.688926815)(29,8.473807009)(30,8.366534389)(31,8.358534201)(32,8.182396103)(33,8.396462811)(34,8.271012892)(35,8.415828848)(36,8.167897335)(37,8.25534914)(38,8.181384558)(39,8.027670786)(40,8.060003098)(41,7.99971981)(42,7.990061356)(43,7.941530552)(44,7.85889572)(45,7.919655016)(46,7.905162687)(47,8.018190882)(48,7.85454203)(49,7.855816732)(50,7.799603132)};\addlegendentry{HC standard val loss}
\addplot[red]coordinates{(1,255.3146145)(2,27.95900442)(3,18.31181137)(4,16.39055273)(5,15.20779941)(6,14.19740698)(7,13.37207154)(8,12.64206936)(9,12.04604232)(10,11.44196109)(11,11.02513553)(12,10.63415717)(13,10.34436429)(14,10.06415156)(15,9.785490496)(16,9.599512872)(17,9.4151847)(18,9.25124012)(19,9.087143952)(20,8.936665181)(21,8.782586605)(22,8.718717793)(23,8.661535299)(24,8.496182178)(25,8.431155521)(26,8.300500657)(27,8.197329659)(28,8.124784009)(29,8.060078628)(30,8.010967848)(31,7.981127901)(32,7.857996452)(33,7.770133211)(34,7.708007798)(35,7.665074913)(36,7.609768813)(37,7.605236831)(38,7.560359192)(39,7.520371384)(40,7.475305292)(41,7.444159162)(42,7.398214444)(43,7.385829746)(44,7.321723127)(45,7.324325357)(46,7.281551455)(47,7.264726968)(48,7.2326907)(49,7.239353021)(50,7.188108735)
};\addlegendentry{loss of SE-PRE}
%\addplot[red,dashed]coordinates{(1,46.85067352)(2,41.90627698)(3,113.6842011)(4,66.81267617)(5,19.23694948)(6,14.2535718)(7,26.92453368)(8,12.5403826)(9,11.97699835)(10,11.64738649)(11,11.71448803)(12,11.08355352)(13,10.57902687)(14,10.29002868)(15,10.05079247)(16,10.43680592)(17,9.994612026)(18,9.745109104)(19,9.801051912)(20,9.52851997)(21,9.20885792)(22,9.296083986)(23,9.393848408)(24,9.31115346)(25,8.986179256)(26,9.020872484)(27,8.919367996)(28,8.789864496)(29,8.756568844)(30,8.890063324)(31,8.754691481)(32,8.614013309)(33,8.57510746)(34,8.486652939)(35,8.420117128)(36,8.354320625)(37,8.392999298)(38,8.374381575)(39,8.284394434)(40,8.393354391)(41,8.197058191)(42,8.397195877)(43,8.370758383)(44,8.14978912)(45,8.139622906)(46,8.124177055)(47,8.136123247)(48,8.113796421)(49,8.047958149)(50,8.019633734)};\addlegendentry{HC pre val loss}
\addplot[blue]coordinates{(1,264.8061946)(2,28.7521678)(3,18.82318241)(4,17.23244495)(5,16.17897792)(6,15.44333299)(7,14.74915674)(8,14.08886853)(9,13.48741767)(10,12.97578842)(11,12.52332146)(12,12.12831274)(13,11.74040393)(14,11.43977499)(15,11.07040893)(16,10.83877219)(17,10.60268841)(18,10.32508724)(19,10.09085365)(20,9.932103477)(21,9.770825149)(22,9.581551394)(23,9.455637853)(24,9.3704919)(25,9.170350541)(26,9.085107474)(27,8.926919662)(28,8.814437881)(29,8.762278944)(30,8.649891763)(31,8.571825632)(32,8.514846562)(33,8.399985339)(34,8.324478778)(35,8.267437839)(36,8.165272445)(37,8.080903234)(38,8.011588526)(39,7.934349906)(40,7.870824179)(41,7.807359677)(42,7.793145966)(43,7.683891885)(44,7.655667635)(45,7.609547111)(46,7.570819987)(47,7.545572116)(48,7.490602284)(49,7.441096358)(50,7.407082539)};\addlegendentry{loss of SE-Identity}
\addplot[orange]coordinates{(1,260.546094)(2,27.55126334)(3,18.68471213)(4,16.84290553)(5,15.76975086)(6,14.8353911)(7,14.13179376)(8,13.52979221)(9,13.00809115)(10,12.50434768)(11,12.09450333)(12,11.74126958)(13,11.36173982)(14,11.07000157)(15,10.7840254)(16,10.55237907)(17,10.30614998)(18,10.09999409)(19,9.933359726)(20,9.760630831)(21,9.557986649)(22,9.461992887)(23,9.293235519)(24,9.166584313)(25,9.039111848)(26,8.907204584)(27,8.808890323)(28,8.733564258)(29,8.630111975)(30,8.559798042)(31,8.450267491)(32,8.387168056)(33,8.267005898)(34,8.145155313)(35,8.125805241)(36,8.072470284)(37,8.036950649)(38,7.952647068)(39,7.888380086)(40,7.893282775)(41,7.823008168)(42,7.749308342)(43,7.731199059)(44,7.696206923)(45,7.6636727)(46,7.593042107)(47,7.599509333)(48,7.532048472)(49,7.522096642)(50,7.475368393)};\addlegendentry{loss of SE-POST}\end{axis}
\end{tikzpicture}
\caption{Progress of training loss for various SE block placing variants. The marked lines are computed as the mean from five runs.}
\label{fig-graph-se-type}
\end{figure}




==> sections/graph_nr_of_anchors.tex <==
\noindent
\begin{figure*}[!h]
\vspace{5mm}
\small
\begin{tikzpicture}
      \begin{axis}[
        height=35mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Number of anchors},
        ymin=0,
        ymax=12,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={1, 3, 6, 9, 12, 15, 18},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(1,7.1)(3,6.9)(6,6.8)(9,6.9)(12,7.0)(15,7.0)(18,7.2)};\addlegendentry{Loss~~~~}
        \addplot[fill=orange!40!white]coordinates{(1,8.2)(3,8.0)(6,7.7)(9,7.8)(12,8.0)(15,7.9)(18,8.0)};\addlegendentry{Val loss}
      \end{axis}
    \end{tikzpicture}
~
 \begin{tikzpicture}
      \begin{axis}[
        height=35mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Number of anchors},
        ymin=0,
        ymax=0.1,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={1, 3, 6, 9, 12, 15, 18},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(1,0.064)(3,0.052)(6,0.069)(9,0.069)(12,0.071)(15,0.062)(18,0.051)};\addlegendentry{Box mAP~~~~}
        \addplot[fill=orange!40!white]coordinates{(1,0.057)(3,0.047)(6,0.063)(9,0.062)(12,0.064)(15,0.057)(18,0.047)};\addlegendentry{Mask mAP}
      \end{axis}
    \end{tikzpicture}
    \vspace{-3mm}
\caption{Left: Dependence of number of anchors on loss. Right: Dependence of number of anchors on mAP. Here, 24 vertices are used.}
\label{graph-nr-anchors}
\end{figure*}

==> sections/graph_nr_of_vertices.tex <==
\noindent
\begin{figure*}[!h]
\small
\begin{tikzpicture}
      \begin{axis}[
        height=39mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Maximal number of vertices per polygon},
        ymin=0,
        ymax=12,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={8, 12, 18, 24, 36, 60, 90},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(8,5.4)(12,5.8)(18,6.5)(24,6.9)(36,7.7)(60,8.8)(90,9.6)};\addlegendentry{Loss~~~~}
        \addplot[fill=orange!40!white]coordinates{(8,6.5)(12,6.9)(18,7.5)(24,7.8)(36,8.5)(60,9.5)(90,10.3)};\addlegendentry{Val loss}
      \end{axis}
    \end{tikzpicture}
~
\begin{tikzpicture}
      \begin{axis}[
        height=39mm,width=99mm,
        ybar,
        enlargelimits=0.07,
        xlabel={Number of anchors},
        ymin=0,
        ymax=12,
        axis x line*=bottom,
        axis y line*=left,
        symbolic x coords={1, 3, 6, 9, 12, 15, 18},
        xtick=data,
        nodes near coords, 
    	nodes near coords align={vertical},
        x tick label style={rotate=0,anchor=center, font=\footnotesize},
        every node near coord/.append style={font=\footnotesize},
        legend style={at={(0.5,1.1)},anchor=north,  font=\footnotesize,nodes={scale=0.9, transform shape}},legend columns=2,
        ]
        \addplot[fill=blue!40!white]coordinates{(1,7.1)(3,6.9)(6,6.8)(9,6.9)(12,7.0)(15,7.0)(18,7.2)};\addlegendentry{Loss~~~~}
        \addplot[fill=orange!40!white]coordinates{(1,8.2)(3,8.0)(6,7.7)(9,7.8)(12,8.0)(15,7.9)(18,8.0)};\addlegendentry{Val loss}
      \end{axis}
    \end{tikzpicture}
    \vspace{-3mm}
\caption{Left: Dependence of number of vertices on loss for 9 used anchors. Right: Dependence of number of anchors on loss for 24 used vertices.}
\label{graph-nr-vertices}
\end{figure*}

==> sections/graph_se_type.tex <==
\noindent
\begin{figure}[!h]
\begin{tikzpicture}
\small
\begin{axis}[height=40mm,width=98mm,xlabel={Epoch},xmin=10, xmax=50, ymin=6.7,ymax=13,legend style={at={(0.79,1)},anchor=north, nodes={scale=0.9, transform shape}},legend columns=1, ymajorgrids=true,yminorgrids=true,style={ultra thick},axis x line*=bottom, axis y line*=left, legend cell align={left}]
\addplot[green]coordinates{(1,269.1180581)(2,28.21265573)(3,18.40226598)(4,16.42302675)(5,15.21275809)(6,14.13723531)(7,13.14906785)(8,12.39609316)(9,11.69206872)(10,11.11319239)(11,10.64653439)(12,10.21312326)(13,9.90192655)(14,9.567035707)(15,9.401223558)(16,9.163649295)(17,8.925355853)(18,8.807712996)(19,8.657624128)(20,8.591970632)(21,8.452182244)(22,8.28339433)(23,8.239628017)(24,8.149788473)(25,8.107046533)(26,7.95557965)(27,7.836849302)(28,7.81011553)(29,7.697173212)(30,7.641633639)(31,7.646899995)(32,7.605880239)(33,7.543636947)(34,7.46002098)(35,7.466055063)(36,7.349977418)(37,7.27898359)(38,7.269490557)(39,7.147420347)(40,7.09822743)(41,7.108537794)(42,7.081504741)(43,7.037955232)(44,7.043813616)(45,7.017336998)(46,7.006936838)(47,6.996316055)(48,6.937507799)(49,6.924841831)(50,6.897511486)};\addlegendentry{loss of SE-Standard}
%\addplot[green,dashed]coordinates{(1,47.50182178)(2,30.68728327)(3,19.68424953)(4,18.29376094)(5,15.03333042)(6,15.33791863)(7,12.89367659)(8,12.2843216)(9,11.94397123)(10,11.56019573)(11,10.73157223)(12,10.5044645)(13,10.12754359)(14,10.38881053)(15,9.809634464)(16,9.612795427)(17,9.718599434)(18,9.197471745)(19,9.753666145)(20,9.072291718)(21,9.236122705)(22,8.766421022)(23,8.788898129)(24,8.958717487)(25,9.128627947)(26,8.551600418)(27,8.563221022)(28,8.688926815)(29,8.473807009)(30,8.366534389)(31,8.358534201)(32,8.182396103)(33,8.396462811)(34,8.271012892)(35,8.415828848)(36,8.167897335)(37,8.25534914)(38,8.181384558)(39,8.027670786)(40,8.060003098)(41,7.99971981)(42,7.990061356)(43,7.941530552)(44,7.85889572)(45,7.919655016)(46,7.905162687)(47,8.018190882)(48,7.85454203)(49,7.855816732)(50,7.799603132)};\addlegendentry{HC standard val loss}
\addplot[red]coordinates{(1,255.3146145)(2,27.95900442)(3,18.31181137)(4,16.39055273)(5,15.20779941)(6,14.19740698)(7,13.37207154)(8,12.64206936)(9,12.04604232)(10,11.44196109)(11,11.02513553)(12,10.63415717)(13,10.34436429)(14,10.06415156)(15,9.785490496)(16,9.599512872)(17,9.4151847)(18,9.25124012)(19,9.087143952)(20,8.936665181)(21,8.782586605)(22,8.718717793)(23,8.661535299)(24,8.496182178)(25,8.431155521)(26,8.300500657)(27,8.197329659)(28,8.124784009)(29,8.060078628)(30,8.010967848)(31,7.981127901)(32,7.857996452)(33,7.770133211)(34,7.708007798)(35,7.665074913)(36,7.609768813)(37,7.605236831)(38,7.560359192)(39,7.520371384)(40,7.475305292)(41,7.444159162)(42,7.398214444)(43,7.385829746)(44,7.321723127)(45,7.324325357)(46,7.281551455)(47,7.264726968)(48,7.2326907)(49,7.239353021)(50,7.188108735)
};\addlegendentry{loss of SE-PRE}
%\addplot[red,dashed]coordinates{(1,46.85067352)(2,41.90627698)(3,113.6842011)(4,66.81267617)(5,19.23694948)(6,14.2535718)(7,26.92453368)(8,12.5403826)(9,11.97699835)(10,11.64738649)(11,11.71448803)(12,11.08355352)(13,10.57902687)(14,10.29002868)(15,10.05079247)(16,10.43680592)(17,9.994612026)(18,9.745109104)(19,9.801051912)(20,9.52851997)(21,9.20885792)(22,9.296083986)(23,9.393848408)(24,9.31115346)(25,8.986179256)(26,9.020872484)(27,8.919367996)(28,8.789864496)(29,8.756568844)(30,8.890063324)(31,8.754691481)(32,8.614013309)(33,8.57510746)(34,8.486652939)(35,8.420117128)(36,8.354320625)(37,8.392999298)(38,8.374381575)(39,8.284394434)(40,8.393354391)(41,8.197058191)(42,8.397195877)(43,8.370758383)(44,8.14978912)(45,8.139622906)(46,8.124177055)(47,8.136123247)(48,8.113796421)(49,8.047958149)(50,8.019633734)};\addlegendentry{HC pre val loss}
\addplot[blue]coordinates{(1,264.8061946)(2,28.7521678)(3,18.82318241)(4,17.23244495)(5,16.17897792)(6,15.44333299)(7,14.74915674)(8,14.08886853)(9,13.48741767)(10,12.97578842)(11,12.52332146)(12,12.12831274)(13,11.74040393)(14,11.43977499)(15,11.07040893)(16,10.83877219)(17,10.60268841)(18,10.32508724)(19,10.09085365)(20,9.932103477)(21,9.770825149)(22,9.581551394)(23,9.455637853)(24,9.3704919)(25,9.170350541)(26,9.085107474)(27,8.926919662)(28,8.814437881)(29,8.762278944)(30,8.649891763)(31,8.571825632)(32,8.514846562)(33,8.399985339)(34,8.324478778)(35,8.267437839)(36,8.165272445)(37,8.080903234)(38,8.011588526)(39,7.934349906)(40,7.870824179)(41,7.807359677)(42,7.793145966)(43,7.683891885)(44,7.655667635)(45,7.609547111)(46,7.570819987)(47,7.545572116)(48,7.490602284)(49,7.441096358)(50,7.407082539)};\addlegendentry{loss of SE-Identity}
\addplot[orange]coordinates{(1,260.546094)(2,27.55126334)(3,18.68471213)(4,16.84290553)(5,15.76975086)(6,14.8353911)(7,14.13179376)(8,13.52979221)(9,13.00809115)(10,12.50434768)(11,12.09450333)(12,11.74126958)(13,11.36173982)(14,11.07000157)(15,10.7840254)(16,10.55237907)(17,10.30614998)(18,10.09999409)(19,9.933359726)(20,9.760630831)(21,9.557986649)(22,9.461992887)(23,9.293235519)(24,9.166584313)(25,9.039111848)(26,8.907204584)(27,8.808890323)(28,8.733564258)(29,8.630111975)(30,8.559798042)(31,8.450267491)(32,8.387168056)(33,8.267005898)(34,8.145155313)(35,8.125805241)(36,8.072470284)(37,8.036950649)(38,7.952647068)(39,7.888380086)(40,7.893282775)(41,7.823008168)(42,7.749308342)(43,7.731199059)(44,7.696206923)(45,7.6636727)(46,7.593042107)(47,7.599509333)(48,7.532048472)(49,7.522096642)(50,7.475368393)};\addlegendentry{loss of SE-POST}\end{axis}
\end{tikzpicture}
\caption{Progress of training loss for various SE block placing variants. The marked lines are computed as the mean from five runs.}
\label{fig-graph-se-type}
\end{figure}



